Exact solution for Riemann problems of the shear shallow water model

The shear shallow water model is a higher order model for shallow flows which includes some shear effects that are neglected in the classical shallow models. The model is a non-conservative hyperbolic system which can admit shocks, rarefactions, shear and contact waves. The notion of weak solution is based on a path but the choice of the correct path is not known for this problem. In this paper, we construct exact solution for the Riemann problem assuming a linear path in the space of conserved variables, which is also used in approximate Riemann solvers. We compare the exact solutions with those obtained from a path conservative finite volume scheme on some representative test cases.

==> RPm_Waves_Structure.tex <==
 \begin{figure}[h]
 \begin{center}
  \begin{tikzpicture}[scale=4.20]
 \coordinate (X0) at (   0.00000000     ,   0.00000000     );
 \coordinate (Xm) at (  -1.40129846E-45 ,   0.00000000     );
 \coordinate (Xp) at (   1.40129846E-45 ,   0.00000000     );
 \coordinate (Xn) at (   0.00000000     ,   1.40129846E-45 );
 \coordinate (Xd001) at (  -1.61687970     ,   0.00000000     );
 \coordinate (Xu001) at (  -1.61687970     ,   1.45000005     );
 \coordinate (Xd002) at (  -1.56445384     ,   0.00000000     );
 \coordinate (Xu002) at (  -1.56445384     ,   1.45000005     );
 \coordinate (Xd003) at (  -1.51500678     ,   0.00000000     );
 \coordinate (Xu003) at (  -1.51500678     ,   1.45000005     );
 \coordinate (Xd004) at (  -1.46828258     ,   0.00000000     );
 \coordinate (Xu004) at (  -1.46828258     ,   1.45000005     );
 \coordinate (Xd005) at (  -1.42405391     ,   0.00000000     );
 \coordinate (Xu005) at (  -1.42405391     ,   1.45000005     );
 \coordinate (Xd006) at (  -1.38211858     ,   0.00000000     );
 \coordinate (Xu006) at (  -1.38211858     ,   1.45000005     );
 \coordinate (Xd007) at (  -1.34229493     ,   0.00000000     );
 \coordinate (Xu007) at (  -1.34229493     ,   1.45000005     );
 \coordinate (Xd008) at (  -1.30442047     ,   0.00000000     );
 \coordinate (Xu008) at (  -1.30442047     ,   1.45000005     );
 \coordinate (Xd009) at (  -1.26834857     ,   0.00000000     );
 \coordinate (Xu009) at (  -1.26834857     ,   1.45000005     );
 \coordinate (Xd010) at (  -1.23394716     ,   0.00000000     );
 \coordinate (Xu010) at (  -1.23394716     ,   1.45000005     );
 \coordinate (Xd011) at (  -1.20109665     ,   0.00000000     );
 \coordinate (Xu011) at (  -1.20109665     ,   1.45000005     );
 \coordinate (Xd012) at (  -1.16968858     ,   0.00000000     );
 \coordinate (Xu012) at (  -1.16968858     ,   1.45000005     );
 \coordinate (Xd013) at (  -1.13962424     ,   0.00000000     );
 \coordinate (Xu013) at (  -1.13962424     ,   1.45000005     );
 \coordinate (Xd014) at (  -1.11081374     ,   0.00000000     );
 \coordinate (Xu014) at (  -1.11081374     ,   1.45000005     );
 \coordinate (Xd015) at (  -1.08317518     ,   0.00000000     );
 \coordinate (Xu015) at (  -1.08317518     ,   1.45000005     );
 \coordinate (Xd016) at (  -1.05663335     ,   0.00000000     );
 \coordinate (Xu016) at (  -1.05663335     ,   1.45000005     );
 \coordinate (Xd017) at (  -1.03111947     ,   0.00000000     );
 \coordinate (Xu017) at (  -1.03111947     ,   1.45000005     );
 \coordinate (Xd018) at (  -1.00657034     ,   0.00000000     );
 \coordinate (Xu018) at (  -1.00657034     ,   1.45000005     );
 \coordinate (Xd019) at ( -0.982927799     ,   0.00000000     );
 \coordinate (Xu019) at ( -0.982927799     ,   1.45000005     );
 \coordinate (Xd020) at ( -0.960138083     ,   0.00000000     );
 \coordinate (Xu020) at ( -0.960138083     ,   1.45000005     );
 \coordinate (Xd021) at ( -0.938151836     ,   0.00000000     );
 \coordinate (Xu021) at ( -0.938151836     ,   1.45000005     );
 \coordinate (Xd022) at ( -0.916923344     ,   0.00000000     );
 \coordinate (Xu022) at ( -0.916923344     ,   1.45000005     );
 \coordinate (Xd023) at ( -0.896410108     ,   0.00000000     );
 \coordinate (Xu023) at ( -0.896410108     ,   1.45000005     );
 \coordinate (Xd024) at ( -0.876572669     ,   0.00000000     );
 \coordinate (Xu024) at ( -0.876572669     ,   1.45000005     );
 \coordinate (Xd025) at ( -0.857374907     ,   0.00000000     );
 \coordinate (Xu025) at ( -0.857374907     ,   1.45000005     );
 \coordinate (Xd026) at ( -0.322138071     ,   0.00000000     );
 \coordinate (Xu026) at ( -0.322138071     ,   1.45000005     );
 \coordinate (Xd027) at (   4.08823341E-02 ,   0.00000000     );
 \coordinate (Xu027) at (   4.08823341E-02 ,   1.45000005     );
 \coordinate (Xd028) at (  0.344088137     ,   0.00000000     );
 \coordinate (Xu028) at (  0.344088137     ,   1.45000005     );
 \coordinate (Xd029) at (  0.933582962     ,   0.00000000     );
 \coordinate (Xu029) at (  0.933582962     ,   1.45000005     );
 \coordinate (Xd030) at (  0.949876368     ,   0.00000000     );
 \coordinate (Xu030) at (  0.949876368     ,   1.45000005     );
 \coordinate (Xd031) at (  0.966609538     ,   0.00000000     );
 \coordinate (Xu031) at (  0.966609538     ,   1.45000005     );
 \coordinate (Xd032) at (  0.983802259     ,   0.00000000     );
 \coordinate (Xu032) at (  0.983802259     ,   1.45000005     );
 \coordinate (Xd033) at (   1.00147581     ,   0.00000000     );
 \coordinate (Xu033) at (   1.00147581     ,   1.45000005     );
 \coordinate (Xd034) at (   1.01965249     ,   0.00000000     );
 \coordinate (Xu034) at (   1.01965249     ,   1.45000005     );
 \coordinate (Xd035) at (   1.03835630     ,   0.00000000     );
 \coordinate (Xu035) at (   1.03835630     ,   1.45000005     );
 \coordinate (Xd036) at (   1.05761254     ,   0.00000000     );
 \coordinate (Xu036) at (   1.05761254     ,   1.45000005     );
 \coordinate (Xd037) at (   1.07744837     ,   0.00000000     );
 \coordinate (Xu037) at (   1.07744837     ,   1.45000005     );
 \coordinate (Xd038) at (   1.09789252     ,   0.00000000     );
 \coordinate (Xu038) at (   1.09789252     ,   1.45000005     );
 \coordinate (Xd039) at (   1.11897564     ,   0.00000000     );
 \coordinate (Xu039) at (   1.11897564     ,   1.45000005     );
 \coordinate (Xd040) at (   1.14073050     ,   0.00000000     );
 \coordinate (Xu040) at (   1.14073050     ,   1.45000005     );
 \coordinate (Xd041) at (   1.16319227     ,   0.00000000     );
 \coordinate (Xu041) at (   1.16319227     ,   1.45000005     );
 \coordinate (Xd042) at (   1.18639874     ,   0.00000000     );
 \coordinate (Xu042) at (   1.18639874     ,   1.45000005     );
 \coordinate (Xd043) at (   1.21038997     ,   0.00000000     );
 \coordinate (Xu043) at (   1.21038997     ,   1.45000005     );
 \coordinate (Xd044) at (   1.23520935     ,   0.00000000     );
 \coordinate (Xu044) at (   1.23520935     ,   1.45000005     );
 \coordinate (Xd045) at (   1.26090300     ,   0.00000000     );
 \coordinate (Xu045) at (   1.26090300     ,   1.45000005     );
 \coordinate (Xd046) at (   1.28752148     ,   0.00000000     );
 \coordinate (Xu046) at (   1.28752148     ,   1.45000005     );
 \coordinate (Xd047) at (   1.31511819     ,   0.00000000     );
 \coordinate (Xu047) at (   1.31511819     ,   1.45000005     );
 \coordinate (Xd048) at (   1.34375131     ,   0.00000000     );
 \coordinate (Xu048) at (   1.34375131     ,   1.45000005     );
 \coordinate (Xd049) at (   1.37348390     ,   0.00000000     );
 \coordinate (Xu049) at (   1.37348390     ,   1.45000005     );
 \coordinate (Xd050) at (   1.40438342     ,   0.00000000     );
 \coordinate (Xu050) at (   1.40438342     ,   1.45000005     );
 \coordinate (Xd051) at (   1.43652391     ,   0.00000000     );
 \coordinate (Xu051) at (   1.43652391     ,   1.45000005     );
 \coordinate (Xd052) at (   1.46998525     ,   0.00000000     );
 \coordinate (Xu052) at (   1.46998525     ,   1.45000005     );
 \coordinate (Xd053) at (   1.50485456     ,   0.00000000     );
 \coordinate (Xu053) at (   1.50485456     ,   1.45000005     );
 \coordinate (Xw001) at (  -1.61687970     ,   0.00000000     );
 \coordinate (Xw002) at ( -0.589756489     ,   0.00000000     );
 \coordinate (Xw003) at ( -0.140627861     ,   0.00000000     );
 \coordinate (Xw004) at (  0.192485243     ,   0.00000000     );
 \coordinate (Xw005) at (  0.638835549     ,   0.00000000     );
 \coordinate (Xw006) at (   1.50485456     ,   0.00000000     );
 \draw[red,line width=0.8mm,dashed]  (Xd001) -- (Xu001);
 \draw[red,line width=0.2mm,dashed]  (Xd002) -- (Xu002);
 \draw[red,line width=0.2mm,dashed]  (Xd003) -- (Xu003);
 \draw[red,line width=0.2mm,dashed]  (Xd004) -- (Xu004);
 \draw[red,line width=0.2mm,dashed]  (Xd005) -- (Xu005);
 \draw[red,line width=0.2mm,dashed]  (Xd006) -- (Xu006);
 \draw[red,line width=0.2mm,dashed]  (Xd007) -- (Xu007);
 \draw[red,line width=0.2mm,dashed]  (Xd008) -- (Xu008);
 \draw[red,line width=0.2mm,dashed]  (Xd009) -- (Xu009);
 \draw[red,line width=0.2mm,dashed]  (Xd010) -- (Xu010);
 \draw[red,line width=0.2mm,dashed]  (Xd011) -- (Xu011);
 \draw[magenta,line width=0.8mm]  (Xd012) -- (Xu012);
 \draw (Xu012) node[anchor=south] {    $ \begin{array}{c} \text{ Shock or}\\\text{ Rarefaction } \end{array}   $};
 \draw[red,line width=0.2mm,dashed]  (Xd013) -- (Xu013);
 \draw[red,line width=0.2mm,dashed]  (Xd014) -- (Xu014);
 \draw[red,line width=0.2mm,dashed]  (Xd015) -- (Xu015);
 \draw[red,line width=0.2mm,dashed]  (Xd016) -- (Xu016);
 \draw[red,line width=0.2mm,dashed]  (Xd017) -- (Xu017);
 \draw[red,line width=0.2mm,dashed]  (Xd018) -- (Xu018);
 \draw[red,line width=0.2mm,dashed]  (Xd019) -- (Xu019);
 \draw[red,line width=0.2mm,dashed]  (Xd020) -- (Xu020);
 \draw[red,line width=0.2mm,dashed]  (Xd021) -- (Xu021);
 \draw[red,line width=0.2mm,dashed]  (Xd022) -- (Xu022);
 \draw[red,line width=0.2mm,dashed]  (Xd023) -- (Xu023);
 \draw[red,line width=0.2mm,dashed]  (Xd024) -- (Xu024);
 \draw[red,line width=0.8mm, dashed]  (Xd025) -- (Xu025);
 \draw[blue,line width=0.8mm]  (Xd026) -- (Xu026);
 \draw (Xu026) node[anchor=south] {Shear} ;
 \draw[line width=0.8mm]  (Xd027) -- (Xu027);
 \draw (Xu027) node[anchor=south] {Contact$\;\;$} ;
 \draw[blue,line width=0.8mm]  (Xd028) -- (Xu028);
 \draw (Xu028) node[anchor=south] {Shear} ;
 \draw[red,line width=0.8mm,dashed]  (Xd029) -- (Xu029);
 \draw[red,line width=0.2mm,dashed]  (Xd030) -- (Xu030);
 \draw[red,line width=0.2mm,dashed]  (Xd031) -- (Xu031);
 \draw[red,line width=0.2mm,dashed]  (Xd032) -- (Xu032);
 \draw[red,line width=0.2mm,dashed]  (Xd033) -- (Xu033);
 \draw[red,line width=0.2mm,dashed]  (Xd034) -- (Xu034);
 \draw[red,line width=0.2mm,dashed]  (Xd035) -- (Xu035);
 \draw[red,line width=0.2mm,dashed]  (Xd036) -- (Xu036);
 \draw[red,line width=0.2mm,dashed]  (Xd037) -- (Xu037);
 \draw[red,line width=0.2mm,dashed]  (Xd038) -- (Xu038);
 \draw[red,line width=0.2mm,dashed]  (Xd039) -- (Xu039);
 \draw[magenta,line width=0.8mm]  (Xd040) -- (Xu040);
 \draw (Xu040) node[anchor=south] {    $ \begin{array}{c} \text{ Shock or}\\\text{ Rarefaction } \end{array}   $};
 \draw[red,line width=0.2mm,dashed]  (Xd041) -- (Xu041);
 \draw[red,line width=0.2mm,dashed]  (Xd042) -- (Xu042);
 \draw[red,line width=0.2mm,dashed]  (Xd043) -- (Xu043);
 \draw[red,line width=0.2mm,dashed]  (Xd044) -- (Xu044);
 \draw[red,line width=0.2mm,dashed]  (Xd045) -- (Xu045);
 \draw[red,line width=0.2mm,dashed]  (Xd046) -- (Xu046);
 \draw[red,line width=0.2mm,dashed]  (Xd047) -- (Xu047);
 \draw[red,line width=0.2mm,dashed]  (Xd048) -- (Xu048);
 \draw[red,line width=0.2mm,dashed]  (Xd049) -- (Xu049);
 \draw[red,line width=0.2mm,dashed]  (Xd050) -- (Xu050);
 \draw[red,line width=0.2mm,dashed]  (Xd051) -- (Xu051);
 \draw[red,line width=0.2mm,dashed]  (Xd052) -- (Xu052);
 \draw[red,line width=0.8mm, dashed]  (Xd053) -- (Xu053);
 \draw (Xw001) node[anchor=south east] {$\Large   \begin{array}{c} h_{\lf}\\[2mm] u_{\lf}\\[2mm] v_{\lf}\\[2mm] \Pres_{\lf}\\[2mm]   \R_{12}^{\lf} \\[2mm] \R_{22}^{\lf}  \end{array} $};
 \draw (Xw002) node[anchor=south] {$\Large   \begin{array}{c} h_{*\lf}\\[2mm] u_{*}\\[2mm] v_{*\lf}\\[2mm] \Pres_{*}\\[2mm]   \R_{12}^{*\lf} \\[2mm] \R_{22}^{*\lf}  \end{array} $};
 \draw (Xw003) node[anchor=south] {$\Large   \begin{array}{c} h_{*\lf}\\[2mm] u_{*}\\[2mm] v_{**}\\[2mm] \Pres_{*}\\[2mm]   \R_{12}^{**} \\[2mm] \R_{22}^{**\lf}  \end{array} $};
 \draw (Xw004) node[anchor=south] {$\Large   \begin{array}{c} h_{*\rg}\\[2mm] u_{*}\\[2mm] v_{**}\\[2mm] \Pres_{*}\\[2mm]   \R_{12}^{**} \\[2mm] \R_{22}^{**\rg}  \end{array} $};
 \draw (Xw005) node[anchor=south] {$\Large   \begin{array}{c} h_{*\rg}\\[2mm] u_{*}\\[2mm] v_{*\rg}\\[2mm] \Pres_{*}\\[2mm]   \R_{12}^{*\rg} \\[2mm] \R_{22}^{*\rg}  \end{array} $};
 \draw (Xw006) node[anchor=south west] {$\Large   \begin{array}{c} h_{\rg}\\[2mm] u_{\rg}\\[2mm] v_{\rg}\\[2mm] \Pres_{\rg}\\[2mm]   \R_{12}^{\rg} \\[2mm] \R_{22}^{\rg}  \end{array} $};
   \end{tikzpicture}
   \caption{ Shear Shalow Water(SSW) model : Waves structure of the 1D
     Riemann problem at a given time. Usefull set  of variables  for the computation of  the analytical solution}
   \label{SSW_RPm_Waves}
 \end{center} 
 \end{figure} 

